Design and Analysis of group-sequential clinical trials based on a modestly-weighted log-rank test in anticipation of a delayed separation of survival curves: A practical guidance

A common feature of many recent trials evaluating the effects of immunotherapy on survival is that non-proportional hazards can be anticipated at the design stage. This raises the possibility to use a statistical method tailored towards testing the purported long-term benefit, rather than applying the more standard log-rank test and/or Cox model. Many such proposals have been made in recent years, but there remains a lack of practical guidance on implementation, particularly in the context of group-sequential designs. In this article, we aim to fill this gap. We discuss how the POPLAR trial, which compared immunotherapy versus chemotherapy in non-small-cell lung cancer, might have been re-designed to be more robust to the presence of a delayed effect. We then provide step-by-step instructions on how to analyse a hypothetical realisation of the trial, based on this new design. Basic theory on weighted log-rank tests and group-sequential methods is covered, and an accompanying R package (including vignette) is provided.

==> notes.tex <==
\section*{Notes}

What do we want this paper to achieve? I think it should be mostly a practical guide for designing and conducting a group-sequential version of the modestly weighted log-rank test, possibly with an extension to an adaptive design.

Technically, in terms of performing the hypothesis test, I think the key result is that the weighted log-rank test has an independent increments structure \cite{tsiatis1982repeated}. The only tricky thing is that when designing the study it's hard to predict what the information levels will be, but I think these kind of issues have been explored for Fleming-Harrington tests \cite{hasegawa2014sample}, \cite{jimenez2019properties}.

Where to position the paper, relative to other literature? What I would like to stress is that a group-sequential modestly-weighted test is far simpler to implement than the proposed group sequential max-combo test \cite{roychoudhury2019robust}, and is barely more difficult than planning a group-sequential log-rank test (when you know there will be non-proportional hazards). Clearly, we will also mention that MWLRT has good operating characteristics under a delayed effect scenario.

Structure?

We could start out with the piece-wise exponential assumption. Then, if you were using a standard log-rank test, how do you set up the group sequential design (emphasize that this is actually already quite a lot of work). Then bring in the modestly-weighted test, and hopefully you don't have to change too much.

%%%%% 

What are the steps?

- We might start off thinking about a clinically relevant effect size, and how many events would be required for sufficient sample size, using a working assumption of proportional hazards.

- We also need to have some idea about the event rates, realistic recruitment expectations, dropouts, and how long we would like the study to last.

- Where would we like to place the interim? Probably just in terms of calendar time.

- (Option 1) calculate sample size for group-sequential design assuming PH then tweak to deal with NPH, or (Option 2) directly calculate sample size under NPH. In either case there are trade-offs in terms of study length / sample size /etc. so there will never be a single design, always a list of options.


%%%%%

{\jose
I like the position of this paper relative to other literature. In terms of the structure we could use, could focus on the comparison log-rank vs. modestly weighted log-rank first, since log-rank is the gold-standard. Then, once the idea that designing a trial using the modestly weighted log-rank is barely more difficult than with the log-rank test, we can discuss the comparison between the modestly weighted log-rank test and the Maxcombo test. I agree with you this may be already a lot. Sample size reassessment could be discussed but not implemented here. I have added at the bottom of these notes some questions that we could discuss in the paper.

A potential structure could be:

\begin{enumerate}
    \item Introduction.
    \item Motivating example from a published Novartis trial?
    \item Model and tests.
    \begin{enumerate}
        \item Piece-wise exponential model.
        \item Log-rank.
        \item Modestly weighted log-rank test.
    \end{enumerate}
    \item Designing a group sequential trial.
    \begin{enumerate}
        \item Simulation set-up (effect size, dropout rate, interim analysis, other assumptions.) Based on a published Novartis trial?. 
        \item Sample size using log-rank.
        \item Sample size using modestly weighted log-rank.
        \item Rejection boundaries and type-I error control.
    \end{enumerate}
    \item Comparison with the Maxcombo test.
    \item Discussion.
\end{enumerate}

\vspace{0.5cm}

\textbf{Questions to discuss}:

\begin{itemize}
    \item When to place the interim analysis?
    \item Sample size reassessment?
    \item Treatment effect quantification?
    \item Comparison of modestly weighted log-rank with test based on restricted mean survival time?
    \item Other non-proportional hazards patterns? (i.e., crossing hazards and decreasing effects).
\end{itemize}

}




%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

We assume that we accrue patients during time $T$ at a constant rate. The total study duration can be defined as $T + \tau$, where $\tau$ represent the time that patients are followed. Following \cite{lakatos1988sample}, the entire study period can be partitioned into $M$ subintervals $\left \{ t_0 = 0, t_1, t_2, \dots, t_M = T + \tau \right \}$.

Let $N_i(j)$ denote the number of patients at risk at time $t_j$, $j = 0, \dots, M-1$. In each subinterval $[t_j, t_{j+1})$, the conditional probability of death for a patient in group $i$ can be approximated by $h_i(t_j) / b$, where $b$ represents the number of subintervals per time unit.

We are assuming a uniform accrual, and therefore the probability of being censored in each subinterval can be approximated by
\begin{equation*}
\left\{\begin{matrix}
1/[b(T+\tau - t_j)] & t_j > \tau\\ 
0 & t_j \leq \tau
\end{matrix}\right.
\end{equation*}

To allow for unequal sample sizes, let $\omega_i$ be the proportion of patients that is planned to be assigned to group $i$. We now define
\begin{equation}
\begin{split}
& N_i(0) = n \omega_i, \\
& N_i(j+1) = N_i(j) \left [ 1 - h_i(t_j) \left ( \frac{1}{b} \right ) - \left ( \frac{1}{b(T + \tau - t_j)} \right ) 1_{\{ t_j > \tau \}} \right ],
\end{split}
\end{equation}where $n$ refers to the total sample size. The expected number of events in each subinterval $[t_j, t_{j+1})$ is then defined as
%
\begin{equation}
D_j = \frac{1}{b} \left ( h_0(t_j) N_0(j) + h_1(t_j)N_1(j) \right ).
\end{equation}
%
It is possible to show that equation \eqref{eq_weighted_logrank_original} can be re-written as
\begin{equation}
E(U) = \frac{\sum_{j=0}^{M-1} D_j^*w_j \left ( \frac{ \left (\frac{N_1(t_j)}{N_0(t_j)} \right ) \cdot \left ( \frac{h_1(t_j)}{h_0(t_j)} \right ) }{1+ \left ( \frac{N_1(t_j)}{N_0(t_j)} \right ) \cdot \left ( \frac{h_1(t_j)}{h_0(t_j)} \right ) } - \frac{\frac{N_1(t_j)}{N_0(t_j)}}{1 + \frac{N_1(t_j)}{N_0(t_j)}} \right )}{\sqrt{\sum_{j=0}^{M-1} D_j^* w_j^2 \left ( \frac{\frac{N_1(t_j)}{N_0(t_j)}}{\left ( 1 + \frac{N_1(t_j)}{N_0(t_j)} \right )^2} \right ) }},
\end{equation}with $w_j = 1$, $j = 1, \dots, M-1$, since we are considering the standard log-rank test. We aim for a power equal to 1 - $\beta$ and a one-sided significance level $1 - \Phi(x_2) = 1 - \Phi(2.01) \approx 0.022$, that already takes into account the actual correlation between $\theta_1$ and $\theta_2$. Since $Z \sim N(\sqrt{n} \cdot E(U), 1)$, we have that 

\begin{equation}
\left | \sqrt{n} \cdot E(U) \right | = (1 - \Phi(x_2)) + z_\beta \Rightarrow n = \left ( \frac{(1 - \Phi(x_2)) + z_\beta}{E(U)} \right )^2.
\end{equation}


%5%%%

\subsection{Type-I error control}
\label{SC_GSD_LR_TYPE1ERROR}

The MONALEESA-7 trial would yield the sequence of standardized test statistics $\textbf{Z} = \{Z_1, Z_2,Z_3\}$. Following \cite{jennison1999group}, these statistics have the null joint distribution

\begin{equation}
\label{eq_canonical_joint1}
\textbf{Z} \sim N({\boldsymbol \mu}, {\boldsymbol \Sigma}),
\end{equation}where 
\begin{equation}
\label{eq_canonical_joint2}
{\boldsymbol \mu} = \begin{pmatrix}
0\\
0\\
0
\end{pmatrix}
\quad
\mbox{and}
\quad
{\boldsymbol \Sigma} = \begin{pmatrix}
1 & \sqrt{\frac{i_1}{i_2}} & \sqrt{\frac{i_1}{i_3}} \\ 
\sqrt{\frac{i_1}{i_2}} & 1 & \sqrt{\frac{i_2}{i_3}} \\
\sqrt{\frac{i_1}{i_3}} & \sqrt{\frac{i_2}{i_3}} & 1 \\
\end{pmatrix},
\end{equation}with $(i_1, i_2, i_3)$ representing the information levels at each look and calculated as
\begin{equation}
\label{eq_information_levels}
i_1 = \frac{\sum_{j=1}^{d_{\tiny \mbox{int}_1}} w_j^2}{\sum_{j=1}^{d_{\tiny \mbox{final}}} w_j^2},
\quad
i_2 = \frac{\sum_{j=1}^{d_{\tiny \mbox{int}_2}} w_j^2}{\sum_{j=1}^{d_{\tiny \mbox{final}}} w_j^2},
\quad
\mbox{and}
\quad
i_3 = \frac{\sum_{j=1}^{d_{\tiny \mbox{final}}} w_j^2}{\sum_{j=1}^{d_{\tiny \mbox{final}}} w_j^2}.
\end{equation}

One fundamental assumption is that, as the group sequential test progresses, the value of the information level $i_k$ is not influenced by the values of $\{Z_1, \dots, Z_{k-1}\}$. The violation of this assumption would destroy the the properties defined in equations \eqref{eq_canonical_joint1} and \eqref{eq_canonical_joint2} on which error rate calculations are based. However, with the (unweighted) log-rank test and assuming the sample size is not reassessed at any interim look, this assumption would not be violated. Then, using the rejection boundaries presented in Table \ref{table_obrien_flemming_boundaries_monaleesa7}, we know that

\begin{equation}
    P(-\infty < Z_1 \leq 3.5950, -\infty < Z_2 \leq 2.3198, -\infty < Z_3 \leq 2.0151) = 0.025.
\end{equation}

In \texttt{R}, the type-I error when using the log-rank test, can be calculated as follows:

<<chunk1>>=
library(mvtnorm)

set.seed(12345)

i1 = 89/252; i2 = 192/252; i3 = 252/252

Sigma = diag(3)
Sigma[1,2] = Sigma[2,1] = sqrt(i1/i2)
Sigma[1,3] = Sigma[3,1] = sqrt(i1/i3)
Sigma[2,3] = Sigma[3,2] = sqrt(i2/i3)
  
typeIerror = 1 - pmvnorm(upper=c(3.5950, 2.3198, 2.0151),sigma=Sigma)[1]

cat("Type-I error:",typeIerror,"\n")

@

\subsection{Sample size calculation}
\label{SC_GSD_LR_SAMPLE_SIZE}

There are several approaches when it comes to calculate the sample size in a delayed effects scenario. We may just start by simply ignoring the delayed effect at the model level, and use a very simple and common working assumption: exponential survival distributions with medians $m_0$ and $m_1$, for the control and experimental treatment groups, respectively. In this case, for 1:1 randomization, the required number of events using the standard log-rank test to achieve a power of $1-\beta$ and assuming a one-sided significance level of $\alpha$ would be
\begin{equation*}
n = 4 \left (\frac{\Phi^{-1}(1 - \beta) + \Phi^{-1}(1-\alpha)}{-\log(m_0/m_1)} \right )^2,
\end{equation*}with a hazard ratio point estimate equal to $\hat{\theta} = \exp \left ( \Phi^{-1}(\alpha) \sqrt{4/n} \right )$. As pointed out by \cite{magirr2020non}, there is a trade-off between $n$ and $\hat{\theta}$ since we may need a larger $n$ to have sufficient power and account for the impact of the delayed effects. However, making $n$ too large would make $\hat{\theta}$ goes to 1, which could lead to getting a significant but not clinically meaningful result. Another issue with this simple approach is the hazard ratio itself since, under non-proportional hazards, the hazard ratio should be interpreted as an average hazard ratio (see e.g., \cite{schemper2009estimation, jimenez2020quantifying}), which does not have a straightforward clinical interpretation. Therefore, finding the right balance between statistical significance and clinical relevance is fairly complex.

An alternative approach includes using more realistic time-to-event distributions. For example, the piece-wise exponential distribution defined in section \ref{sc_pieceweise_exponential_model} allows to incorporate the delayed effect assumption into the working model. This would allow to empirically calculate the required number of events to achieve a power of $1-\beta$ assuming a one-sided significance level of $\alpha$ as follows:

\begin{enumerate}[label=\roman*)]
    \item Fix the number of events $n$ (e.g., $n = 100$).
    \item Simulate $M$ trials, each with $n$ events, and calculate at the end of each trial $I (Z > \Phi^{-1}(1-\alpha))$, where $Z$ is the standardized log-rank test statistic.
    \item Calculate the empirical power for a fixed number of events as 
    \begin{equation}
    \label{eq_empirical_power}
    \widehat{\mbox{Power}} = \frac{1}{M} \sum_{i = 1}^{M} I (Z > \Phi^{-1}(1-\alpha)).
    \end{equation}
    
    \item Repeat steps ii) and iii) adjusting $n$ until \eqref{eq_empirical_power} yields a value equal to $1-\beta$.
\end{enumerate}

This iterative procedure, that has also been formalized in a sample size formula (see \cite{lakatos1988sample, hasegawa2014sample}), would guarantee a more realistic power for the log-rank test since the delayed effects assumption is already taken into account through the piece-wise exponential distributions defined in section \ref{sc_pieceweise_exponential_model}. It should be taken into consideration however that log-rank test is not the most powerful test under delayed effects (see e.g., \cite{jimenez2019properties}). Therefore, by using a weighted log-rank test (see sections \ref{SC_GSD_WLR} and \ref{SC_GSD_MAXCOMBO}), we could significantly reduce the sample size. However, the balance between statistical significance and clinical relevance would still remain as an issue since the hazard ratio lacks clinical interpretability.

The MONALEESA-7 trial assumed that the control and experimental groups had OS medians of 33 and 47 months, respectively. Under these assumptions, the trial required 252 events to achieve a power of 80\%, as explained in section \ref{SC_MONALEESA}, and no potential delayed effect was ever taken into account. However, as presented in \cite{im2019overall} (Figure 1A), there was a delayed effect of approximately 20 months, which rendered the trial under-powered. 

In Figure \ref{figure_sample_size_gsd_logrank}, we present the empirically estimated power and the correspondent required number of events for different delays using the standard log-rank test. Results show that, as the delay increases, the required number events necessary to guarantee a power of 80\% using the standard log-rank test becomes unfeasible.

\begin{figure}[t]
  \centering
   \caption{Empirically estimated power and corresponding number of events for different delay values based on the initial assumptions made by the MONALEESA-7 trial.}
   \vspace{0.5cm}
  \includegraphics[scale=0.65]{Figures/sample_size_gsd_logrank.pdf}
  \label{figure_sample_size_gsd_logrank}
\end{figure}

Outside of the log-rank (and weighted log-rank) test, we believe that alternative methods such us the robust milestone (or landmark) analysis or the restricted mean survival time (RMST), should be taken more into consideration as they allow to find the balance between statistical significance and clinical relevance since they are always clinically interpretable. In fact, it is possible to show that standard log-rank and RMST achieve very similar power values (see e.g., \cite{jimenez2020quantifying}).

\section{Group-sequential weighted log-rank test}
\label{SC_GSD_WLR}

\subsection{Type-I error control}
\label{SC_GSD_WLR_TYPE1ERROR}

As pointed out by \cite{jennison1999group,jimenez2020response}, the joint distribution defined in \eqref{eq_canonical_joint1} and \eqref{eq_canonical_joint2} holds if the correlation between two test statistics $Z_1$ and $Z_2$ is equal to $\sqrt{i_1 / i_2} = \sqrt{d_{\tiny \mbox{int}_1} / d_{\tiny \mbox{int}_2}}$. As discussed in section \ref{SC_GSD_LR_TYPE1ERROR}, this assumption holds with the log-rank test because $w=1$. However, it is straightforward to see that with any weighted log-rank test, $\sqrt{i_1 / i_2} \neq \sqrt{d_{\tiny \mbox{int}_1} / d_{\tiny \mbox{int}_2}}$ because some event time are down-weighted. Therefore, rejection boundaries should be recalculated by accounting for the actual correlation between test statistics. To do that in this kind of setting with 3 looks to the data, we would calculate the rejection boundaries in the following two-step procedure, assuming the ``cumulative $\alpha$ spent''  from Table \ref{table_obrien_flemming_boundaries_monaleesa7}:

\begin{enumerate}[label=\roman*)]
    \item Calculate the rejection boundary for the interim analysis number 2 based on the correlation between between the test statistics from interim analyses 1 and 2.
    
    \begin{equation}
    f(\mbox{\textbf{x}}) = \frac{1}{2\pi}(\mbox{det } \Sigma)^{\frac{1}{2}} \int_{-\infty}^{x_{\tiny \mbox{int}_2}} \int_{-\infty}^{x_{\tiny \mbox{int}_1}} \exp \left ( -\frac{1}{2} (\mbox{\textbf{x}} - {\boldsymbol \mu})^{T} {\boldsymbol \Sigma}^{-1} (\mbox{\textbf{x}} - {\boldsymbol \mu}) \right ) d\mbox{\textbf{x}},
    \end{equation}where $\Sigma = \begin{pmatrix}
1 & \sqrt{i_1 / i_2} \\ 
\sqrt{i_1 / i_2} & 1
\end{pmatrix}$.
    
    We numerically find the value of $x_{\tiny \mbox{int}_2}$ using the following piece of \emph{R} code placed below. In this code, we search for a value of $x_{\tiny \mbox{int}_2}$ that is a root (i.e., zero) of the function \texttt{crit\_adj(y, alpha1 = 0.00016221, alpha = 0.01023316, corr = ((1-$\rho$)*diag(2) + $\rho$))} within the interval [0,3]. The value of $x_{\tiny \mbox{int}_2}$ will correspond to the rejection boundary for the interim analysis number 2.
    
    \item Calculate the rejection boundary for the final analysis based on the correlation between between the test statistics from interim analysis 2 and final analysis.
    
    \begin{equation}
    f(\mbox{\textbf{x}}) = \frac{1}{2\pi}(\mbox{det } \Sigma)^{\frac{1}{2}} \int_{-\infty}^{x_{\tiny \mbox{final}}} \int_{-\infty}^{x_{\tiny \mbox{int}_2}} \exp \left ( -\frac{1}{2} (\mbox{\textbf{x}} - {\boldsymbol \mu})^{T} {\boldsymbol \Sigma}^{-1} (\mbox{\textbf{x}} - {\boldsymbol \mu}) \right ) d\mbox{\textbf{x}},
\end{equation}where $\Sigma = \begin{pmatrix}
1 & \sqrt{i_2 / i_3} \\ 
\sqrt{i_2 / i_3} & 1
\end{pmatrix}$.

We numerically find the value of $x_{\tiny \mbox{final}}$ using the following piece of \emph{R} code placed in the appendix. In this code, we search for a value of $x_{\tiny \mbox{final}}$ that is a root (i.e., zero) of the function \texttt{crit\_adj(y, alpha1 = 0.01023316, alpha = 0.025, corr = ((1-$\rho$)*diag(2) + $\rho$))} within the interval [0,3]. The value of $x_{\tiny \mbox{final}}$ will correspond to the rejection boundary for the interim analysis number 2.

\end{enumerate}

\subsection{Sample size calculation}
\label{SC_GSD_WLR_SAMPLE_SIZE}

To calculate the required sample size for a group sequential test using the weighted log-rank, we go back to the iterative procedure defined in section \ref{SC_GSD_LR_SAMPLE_SIZE} or to the sample size formula derived by \cite{hasegawa2014sample}. In this context, we explore the performance of two weighted log-rank tests: the Fleming and Harrington class of weights proposed by \cite{fleming1981class}, and the modestly weighted log-rank test proposed by \cite{magirr2019modestly}. 

Using the Fleming and Harrington class of weights, we may choose from many parameter combinations depending on the events we want to down-weight. Under delayed effects and following \cite{jimenez2019properties}, we consider the combination $(\rho=0, \gamma=1)$ which aims to down-weight early events. In Figure \ref{sample_size_gsd_weightedlogrank}, we present the empirically estimated power and the correspondent required number of events for different delays using the weighted log-rank test with the Fleming and Harrington class of weights $G_{(\rho=0, \gamma=1)}$. We observe a notable difference if using the standard log-rank test or using $G_{(\rho=0, \gamma=1)}$. For instance, using the standard log-rank test, with 250 events and delays of 2, 4 and 8 months, the estimated power presented in Figure \ref{figure_sample_size_gsd_logrank} is close to 52\%, 28\% and 8\%, respectively. However, using the Fleming and Harrington class of weights $G_{(\rho=0, \gamma=1)}$, with 300 events and delays of 2, 4 and 8 months, the estimated power is close to 65\%, 62\% and 50\%, respectively. These power values translate into relative efficiencies of $G_{(\rho=0, \gamma=1)}$ with respect to the standard log-rank test of 138\%, 271\% and 1402\%, respectively.

\begin{figure}[t]
  \centering
   \caption{Empirically estimated power and corresponding number of events for different delay values based on the initial assumptions made by the MONALEESA-7 trial.}
   \vspace{0.5cm}
  \includegraphics[scale=0.65]{Figures/sample_size_gsd_weightedlogrank_fh.pdf}
  \label{sample_size_gsd_weightedlogrank}
\end{figure}

\begin{figure}[t]
  \centering
   \caption{Empirically estimated power and corresponding number of events for different delay values based on the initial assumptions made by the MONALEESA-7 trial.}
   \vspace{0.5cm}
  \includegraphics[scale=0.6]{Figures/sample_size_gsd_weightedlogrank_magirr.pdf}
  \label{sample_size_gsd_weightedlogrank_magirr}
\end{figure}


\section{Group-sequential max-combo test}
\label{SC_GSD_MAXCOMBO}


\section{Case study: Revisiting the MONALEESA-7 trial}
\label{SC_MONALEESA}

In this section we introduce the MONALEESA-7 trial \cite{im2019overall}, a case study that we use to create a realistic simulation set-up to implement the methodology described along the manuscript. It is, however, out of the scope of this article to re-analyze it or make new clinical interpretations of its data.

The MONALEESA-7 trial (ClinicalTrials.gov number \texttt{NCT02278120}) is a randomized, double-blind, placebo-controlled, phase 3 trial comparing ribociclib with placebo, in addition to endocrine therapy, in premenopausal or perimenopausal women with hormone-receptor–positive, HER2-negative advanced breast cancer. In this trial, patients were randomly assigned, in a 1:1 ratio, to receive ribociclib (at a dose of 600 mg, administered orally once daily for 21 consecutive days, followed by 7 days off, for a complete cycle of 28 days) or matching placebo. Crossover between the two groups was not permitted.

In this trial, the primary endpoint was PFS whereas OS was specified as a key secondary end point and would be tested only if PFS reached statistical significance. A hierarchical testing strategy between PFS and OS was used to control the family-wise type-I error rate at 2.5\% \cite{glimm2010hierarchical}. 

The sample size was calculated on the basis of the primary end point of PFS where PFS medians of 9 and 13.4 months were assumed for the control and experimental groups, respectively, which translates into a hazard ratio of 0.67. A total of 329 PFS events at a one-sided overall 2.5\% level of significance would provide a 95\% power to reject $H_0$. No interim analyses were planned for PFS.

This study considered a recruitment period of approximately 18 months at a uniform rate of 33 patients/month. Therefore, 600 patients will need to be randomized to the two treatment arms in a 1:1 ratio. Assuming about 10\% patients would be lost to follow-up for PFS, a total of 660 patients needed to be randomized. Given these assumptions, it was estimated that the 329-th PFS event would be observed at approximately 22 months from the date of first patient randomized in the study.

OS medians of 33 and 47 months were assumed for the control and experimental groups, respectively, which translates into a hazard ratio of 0.7. A total of 252 OS events at a one-sided overall 2.5\% level of significance would provide a 80\% power to reject $H_0$ using the standard log-rank test and 3-look group sequential design. It was estimated that these 252 deaths would be observed at approximately 40 months from the date of first patient to be randomized. Therefore the estimated time for the final OS evaluation would be 18 months after the primary analysis of the PFS endpoint has been conducted. The group sequential testing of OS were based on the O'Brien and Fleming boundaries presented in Table \ref{table_obrien_flemming_boundaries_monaleesa7}.

\begin{table}[]
\centering
\caption{O'Brien and Fleming boundaries used for the group sequential analysis of OS in the MONALEESA-7 trial.}
\begin{tabular}{|c|c|c|c|c|}
\hline
\makecell{Interim \\ look} & \makecell{Information \\ fraction} & OS events & \makecell{Cumulative \\ $\alpha$ spent} & \makecell{Efficacy boundaries \\ ($Z$)} \\ \hline
1 & 0.35317 &  89 & 0.00016221 & 3.5950 \\ \hline
2 & 0.76190 & 192 & 0.01023316 & 2.3198 \\ \hline
3 & 1 & 252 & 0.025 & 2.0151 \\ \hline 
\end{tabular}
\label{table_obrien_flemming_boundaries_monaleesa7}
\end{table}

The primary analysis of PFS was conducted after 318 patients had disease progression or had died, where statistical significance was achieved. The first interim analysis of OS was performed after 89 deaths had occurred and the corresponding O'Brien and Fleming boundary (see Table \ref{table_obrien_flemming_boundaries_monaleesa7}) was not crossed. The second interim analysis of OS was performed after 192 deaths had occurred and the corresponding O'Brien and Fleming boundary was crossed. Therefore, statistical significance was achieved and superiority of the experimental group with respect to the control group was claimed.


\section{Discussion}

\bibliographystyle{unsrt}
\bibliography{references}

\clearpage

\newpage

\section*{Appendix}

\subsection*{Independent increments}

Let $\textbf{Z} = (Z_1,Z_2,Z_3)'$ be the (unweighted) log-rank standardized test statistics at the interim and final analyses respectively, under the $H_0$ defined in \eqref{eq_null_hypothesis}. Therefore, $\textbf{Z}$ has the joint distribution

\begin{equation*}
\textbf{Z} \sim N \left (
{\boldsymbol \mu}, {\boldsymbol \Sigma} \right ),
\end{equation*}where 
\begin{equation*}
{\boldsymbol \mu} = \begin{pmatrix}
0\\
0\\
0
\end{pmatrix}
\quad
\mbox{and}
\quad
{\boldsymbol \Sigma} = \begin{pmatrix}
1 & \sqrt{\frac{i_1}{i_2}} & \sqrt{\frac{i_1}{i_3}} \\ 
\sqrt{\frac{i_1}{i_2}} & 1 & \sqrt{\frac{i_2}{i_3}} \\
\sqrt{\frac{i_1}{i_3}} & \sqrt{\frac{i_2}{i_3}} & 1 \\
\end{pmatrix},
\end{equation*}with $i_1$, $i_2$ and $i_3$ being the the information fraction after stages 1 and 2 (interim analyses) and stage 3 (final analysis) of the trial. For the unweighted log-rank test, under the null hypothesis, $i_1 = \frac{d_1}{4}$, $i_2 = \frac{d_2}{4}$ and $i_3 = \frac{d_3}{4}$, where $d_1$, $d_2$ and $d_3$ are the number of events across both arms after stages 1, 2 and 3 of the trial. Now let 
\begin{equation*}
\begin{split}
& Z' = \frac{\sqrt{i_2} Z_2 - \sqrt{i_1} Z_1}{\sqrt{i_2 - i_1}},\\
& Z'' = \frac{\sqrt{i_3} Z_3 - \sqrt{i_2} Z_2}{\sqrt{i_3 - i_2}},
\end{split}
\end{equation*}and
\begin{equation*}
{\boldsymbol \Omega} = \begin{pmatrix}
1 & 0 & 0 \\ 
- \frac{\sqrt{i_1}}{\sqrt{i_2 - i_1}} & \frac{\sqrt{i_2}}{\sqrt{i_2 - i_1}} & 0 \\
0 & - \frac{\sqrt{i_2}}{\sqrt{i_3 - i_2}} & \frac{\sqrt{i_3}}{\sqrt{i_3 - i_2}}
\end{pmatrix}.
\end{equation*}

By the standard formula for the multivariate Normal distribution (see e.g. \cite{jupp1979maximum}), the joint distribution of ${\boldsymbol \Omega} \times \textbf{Z} \sim N \left ( {\boldsymbol \mu}, I_3 \right )$ since ${\boldsymbol \Omega} \times {\boldsymbol \Sigma} \times {\boldsymbol \Omega}' = I_3$. Thus, $Z'$ and $Z''$ are stochastically independent from $Z_1$ and $Z_2$, respectively, and therefore are referred as ``independent increments''.

\subsection*{Rejection boundaries (R code)}

<<chunk2>>=
library(mvtnorm)
library(gridExtra)

#calculate the critical value
crit_adj = function(z2, alpha1, alpha2, corr){
  z1<-qnorm(1-alpha1)
  rejprob<-1-pmvnorm(upper=c(z1,z2),corr=corr)
  return(rejprob-alpha2)
}
#Correlation between the test statistics of the interim looks 1 and 2:
correlation = sqrt(0.75)
#Variance-covariance matrix:
corr = (1-correlation)*diag(2)+correlation
#Cumulative alpha spent at interim looks 1 and 2
alpha1 = 0.01; alpha2 = 0.025 

#Critical value (i.e., rejection boundary) for interim look number 2 in the z-scale:
crit_final = uniroot(crit_adj, lower = 0, upper = 3, alpha1 = alpha1, 
alpha2 = alpha2, corr = corr, tol = 1E-12)
z = crit_final$root

cat("Rejection boundary look 2:",z,"\n")

@

